Competing Influence in LLM Populations: Budget Timing and Baseline Drift

When competing campaigns target a population of large language model (LLM) agents, observed opinion changes may reflect both campaign influence and changes that would occur without intervention. We study how the timing of campaign expenditure and the population's own evolution shape outcomes in a network of persona-conditioned LLM agents that exchange and revise opinions in natural language. A proponent and a challenger are tasked with generating opposing messages under equal delivery budgets, while a separate stance probe measures opinions without influencing the simulation. Across eight claims, we compare single-campaign and competitive conditions against matched no-campaign runs, and evaluate all nine combinations of early, sustained, and late spending on a reference topic. Baseline stance drift varies substantially across claims and, on some, accounts for a sizeable fraction of apparent campaign effects. After accounting for this drift, the direction of observed campaign-associated changes aligns more closely with the claim's epistemic standing than with the campaigner's assigned role. Uninfluenced populations also consistently lose stance diversity, demonstrating that directional opinion change and convergence are distinct phenomena. In networks with two opinion-segregated communities, campaigns primarily reduce differences between communities rather than diversity within them. LLM campaign agents do not always argue for their assigned positions, particularly when these conflict with established evidence. Finally, campaign outcomes depend on the opponent's expenditure schedule: unlike a matched numerical bounded-confidence population receiving interventions at the same times and locations, the LLM population exhibits a payoff structure with no pure-strategy equilibrium.

==> figures/simulation_setup-old.tex <==

\section{Simulation Setup}
\label{sec:setup}

We simulate a contest between two campaign agents over a population of
persona-conditioned LLM agents. The design has three kinds of component,
and keeping them apart is what the rest of this section is about.

\emph{Agents} act. These are the population agents and the two campaign
agents: a \prop, which argues for the topic claim, and a \chal, which
argues against it. \emph{Measurement models} observe and never act. These
are a stance probe, which converts written positions into numbers for
analysis, and a message rater, which scores campaign messages. No agent
can see either measurement model, and neither model feeds anything back
into the simulation. \emph{Policies} are the strategic object. A policy
fixes how a campaign agent spends its budget across rounds, and the
experiment compares policies against each other.

Two things differ from our earlier formulation~\cite{qasmi2025}, where
the population evolved under a scalar bounded-confidence rule. First,
population beliefs are held and revised in natural language, and the
number used for analysis is produced afterwards by a separate model that
the population never sees. Second, both campaign agents have the same
budget and the same price for reaching people, so any difference in
outcome comes from content and from the population's own dispositions
rather than from the specification.

We name the campaign agents for what they do, not for whether they are
correct. A \prop{} argues for the claim whether or not the claim is true.
As Section~\ref{sec:conditions} explains, the topic set deliberately
includes claims that are false, claims that are contested, and claims
that are well supported, so on some topics it is the \chal{} that argues
the weaker position.

\subsection{Population and Network}
\label{sec:population}

The population is a directed graph $G=(\mathcal{V},\mathcal{E})$ with
$|\mathcal{V}|=N$ agents. Edges come from a directed configuration model
with mean out-degree $\bar{d}$. We write
$\mathcal{N}^{-}(i)=\{j:(j,i)\in\mathcal{E}\}$ for the set of agents
whose posts agent $i$ reads. The graph is fixed for a run and drawn again
for each replicate.

Each agent $i$ gets a persona $p_i$ drawn without replacement from a bank
of demographic and stylistic attributes: an age band, an occupation, a
location, a news-consumption habit, and a writing style. Occupations
carry a minimum age band so that the combinations stay plausible.

Personas carry no attribute relating to opinion or to susceptibility.
Susceptibility is instead represented by two model parameters,
$\lambda$ and $w$, described in Section~\ref{sec:update}. We keep it
there so that it can be reported as a fixed number, rather than being
mixed into the wording of a persona where its effect could not be
separated from the effect of the network.

An agent's belief state at round $t$ is a short written \emph{position}
$s_i^{t}$ of at most $\ell$ tokens. Its first position $s_i^{0}$ is
generated once from the persona and the topic claim, and is kept
unchanged for the rest of the run.

\subsection{Stance Measurement}
\label{sec:measurement}

Analysis needs a number, but asking the agents to supply one would make
the population both the thing being measured and the instrument
measuring it. We separate the two. A stance probe $\Pi$, taken from a
different model family than the population, run at temperature zero and
held fixed across all conditions, maps a position to a number,
\begin{equation}
  x_i^{t} \;=\; \Pi\!\left(s_i^{t}\right) \;\in\; [-1,1],
  \label{eq:probe}
\end{equation}
where $-1$ means the claim is fully rejected and $+1$ means it is fully
accepted.

Positions are written to a log and the probe runs over that log after
the simulation has finished. Two things follow. Measurement adds nothing
to the time taken by a round, and measurement can be repeated or
redefined later without running any simulation again.

We establish how reliable the probe is once, in a separate exercise.
We take $n_{\mathrm{val}}$ logged positions, score each of them
$k_{\mathrm{val}}$ times, and report the intra-class correlation and the
median absolute difference between repeated scores of the same position.
Production measurement then uses one score per position, since the
variability we have just measured belongs to the instrument and not to
any individual reading.

\subsection{Campaign Agents and the Budget Game}
\label{sec:game}

A \prop{} and a \chal{} compete over the population. Both are LLM agents
with role instructions. Both receive the same budget
$B_{\mathrm{P}}=B_{\mathrm{C}}=B$ and face the same prices.

\paragraph{Budget buys reach.}
At round $t$ a side $c\in\{\mathrm{P},\mathrm{C}\}$ spends
$a_c^{t}\in\mathbb{Z}_{\ge0}$ and sends its message to a set
$\mathcal{T}_c^{t}\subseteq\mathcal{V}$ of that size, subject to
\begin{equation}
  \sum_{t=1}^{T} a_c^{t} \;\le\; B ,
  \qquad c\in\{\mathrm{P},\mathrm{C}\} .
  \label{eq:budget}
\end{equation}
One unit of budget delivers one message to one agent. A delivery reaches
a distinct agent, so a round can carry at most $N$ deliveries. A policy
that asks for more is capped at $N$ and the remainder is carried into
the next round rather than lost. We set $B=\tfrac{1}{3}NT$, which is the
largest budget for which the front-loaded policy below is deliverable
without hitting that cap.

The research question concerns when budget is spent, not on whom, so
$\mathcal{T}_c^{t}$ is drawn uniformly at random from $\mathcal{V}$.
Choosing targets by degree, centrality or community membership is
outside the scope of this study; Section~\ref{sec:limitations} says why.

\paragraph{Timing policies.}
A policy is a schedule $\pi_c:\{1,\dots,T\}\to\mathbb{Z}_{\ge0}$ with
$\sum_t \pi_c(t)\le B$. We use three, chosen to cover the early-versus-late
trade-off that Dhamal et al.~\cite{dhamal2020} identify for classical
opinion dynamics:
\begin{align}
  \pi^{\mathrm{front}}(t) &=
    \begin{cases}
      \lfloor 3B/T \rfloor, & t \le \lceil T/3 \rceil,\\
      0, & \text{otherwise},
    \end{cases}
  \label{eq:front}\\[2pt]
  \pi^{\mathrm{unif}}(t)  &= \lfloor B/T \rfloor
    \quad \text{for all } t,
  \label{eq:unif}\\[2pt]
  \pi^{\mathrm{back}}(t)  &=
    \begin{cases}
      \lfloor 3B/T \rfloor, & t > \lfloor 2T/3 \rfloor,\\
      0, & \text{otherwise}.
    \end{cases}
  \label{eq:back}
\end{align}
Rounding leaves a remainder, which is spent in the last active round of
the policy, so all three policies spend exactly $B$. The strategy space
is the $3\times3$ product of policies for the two sides. We treat it as
a normal-form game and report the payoff matrix and its pure-strategy
equilibria.

\paragraph{What the campaign agents can and cannot see.}
Spending is not an agent decision. Each $\pi_c$ is fixed before the run
starts and targets are random. We chose this because a normal-form game
needs strategies that are committed in advance, which is what makes the
payoff matrix and its equilibrium well defined, and because it matches
the two-phase investment game we are comparing against~\cite{dhamal2020}.
The strategic choice in this study is the choice of policy, and the
experiment plays every policy against every other.

What a message says does adapt. In each active round a campaign agent is
shown the information a real campaigner could obtain: the round number
and the length of the campaign, how much of its own budget is left, how
many agents the other side reached in the previous round, its own
previous message, and $n_{s}$ current population posts sampled at random
and given as text.

A campaign agent is never shown a stance value, for any agent or for the
population as a whole. If campaign agents could act on probe output, the
probe would have to run inside every round, and the instrument would
become part of the process it is supposed to measure.

We also implement a fourth, closed-loop policy, \textsc{reactive}, which
sets each round's spending from the other side's observed reach in the
previous round, subject to a pacing limit. It is not a fixed strategy, so
we leave it out of the payoff matrix and report it separately.

\paragraph{Rating campaign messages.}
A message rater $J$ scores every message $m_c^{t}$ on five dimensions,
each between $0$ and $1$: clarity, evidential grounding, relevance,
emotional appeal, and persuasiveness. The rater is asked for each
dimension separately and returns them through a constrained output
schema, so every message has a complete set of scores and nothing has to
be recovered from free text.

We do not combine the five into a single score. Grounding and
persuasiveness come apart in exactly the way that matters here: a false
claim can be persuasive and poorly grounded at the same time, and a
correct rebuttal can be well grounded and unpersuasive. An average would
give those two cases the same value and lose the contrast the analysis
needs. We therefore report all five dimensions separately, broken down by
side.

No rating enters the population update. Message quality is recorded
alongside the simulation, which lets us look at whether opinion movement
tracks measured quality instead of building that relationship into the
model. This is a change from our earlier
formulation~\cite{qasmi2025}, where a rating multiplied the opinion
shift directly.

We check the rater once before the main experiment. We rate a sample of
messages $k_{J}$ times each and report, for every dimension, the spread
between messages, the spread across repeats of the same message, and the
intra-class correlation $\mathrm{ICC}(1,1)$. Dimensions that turn out to
be unreliable are reported as such rather than used. Rating, like stance
measurement, happens after the run.

\subsection{Round Structure and Belief Revision}
\label{sec:update}

A run has $T$ campaign rounds followed by $T'$ quiet rounds in which both
budgets are spent and no campaign messages are sent. The quiet rounds are
where a difference between immediate impact and lasting impact becomes
visible. Without them, a short-lived gain and a durable one look the same.

Within a round, agent $i$ rewrites its position given four inputs: its
persona $p_i$, its current position $s_i^{t}$, the posts of the agents it
follows, and any campaign message addressed to it. Its first position
$s_i^{0}$ is placed back into the prompt with weight $\lambda$, which
acts as a resistance to persuasion and plays the role that retention
plays in Friedkin--Johnsen models~\cite{friedkin1990,he2026}. The
probability $w$ that an addressed agent reads the message it is sent is
fixed at $1$. We report $\lambda$ and $w$ as constants rather than
varying them, because variation in susceptibility is not one of our
research questions.

\begin{algorithm}[t]
\caption{One round of the simulation}
\label{alg:round}
\begin{algorithmic}[1]
\Require positions $\{s_i^{t}\}$, budgets $\{B_c^{t}\}$, policies $\{\pi_c\}$
\For{$c \in \{\mathrm{P},\mathrm{C}\}$ \textbf{in parallel}}
  \State $a_c^{t} \gets \min\!\big(\pi_c(t)+\text{carry}_c,\; B_c^{t},\; N\big)$
  \State $\text{carry}_c \gets \min(\pi_c(t)+\text{carry}_c, B_c^{t}) - a_c^{t}$
  \If{$a_c^{t} > 0$}
    \State $\mathrm{ctx} \gets$ round, budget left, other side's last reach,
    \Statex \hspace{2.2em} own last message, $n_s$ sampled posts
    \State $m_c^{t} \gets \textsc{Generate}(c, \text{claim}, \mathrm{ctx})$
    \State $\mathcal{T}_c^{t} \gets$ sample $a_c^{t}$ agents from $\mathcal{V}$
    \State $B_c^{t+1} \gets B_c^{t} - a_c^{t}$
  \EndIf
\EndFor
\For{$i \in \mathcal{V}$ \textbf{in parallel}}
  \State $M_i \gets \{\, m_c^{t} : i \in \mathcal{T}_c^{t} \,\}$
  \State $s_i^{t+1} \gets \textsc{Revise}\big(p_i,\, s_i^{t},\,
          \{s_j^{t}\}_{j\in\mathcal{N}^{-}(i)},\, M_i,\,
          s_i^{0}\!\mid\!\lambda\big)$
\EndFor
\State \textbf{log} $\{s_i^{t+1}\}$, $\{m_c^{t}\}$, $\{a_c^{t}\}$
\Statex \Comment{stance and message ratings are produced later, from the log}
\end{algorithmic}
\end{algorithm}

\subsection{Numerical Comparison Arm}
\label{sec:bcm}

To tell apart what the allocation problem contributes from what the
population mechanism contributes, we run every campaign condition a
second time on a numerical population, using the same graph, budgets,
policies and horizon. Agents hold a single number and update under a
bounded-confidence rule with a term that pulls them back towards their
starting opinion. Writing
$\mathcal{C}_i^{t}=\{\,j\in\mathcal{N}^{-}(i):
|x_j^{t}-x_i^{t}|\le\varepsilon\,\}$ for the set of neighbours close
enough to be listened to,
\begin{equation}
  \tilde{x}_i^{t}
  = x_i^{t} + \mu\!\left(
      \frac{1}{|\mathcal{C}_i^{t}|}
      \sum_{j\in\mathcal{C}_i^{t}} x_j^{t} - x_i^{t}
    \right),
  \label{eq:bcm-core}
\end{equation}
\begin{equation}
  x_i^{t+1}
  = (1-\lambda)\Big(
      \tilde{x}_i^{t}
      + \eta \!\!\sum_{c:\, i\in\mathcal{T}_c^{t}}\!\! \sigma_c
    \Big)
    + \lambda\, x_i^{0},
  \label{eq:bcm-campaign}
\end{equation}
clipped to $[-1,1]$, where $\sigma_{\mathrm{P}}=+1$,
$\sigma_{\mathrm{C}}=-1$ and $\eta$ sets the size of a campaign's effect.
No message rating appears in Eq.~\eqref{eq:bcm-campaign}, for the same
reason it does not appear in the LLM arm.

Two points of notation. The threshold $\varepsilon$ and the rate $\mu$
are separate parameters here, whereas a single symbol served both
purposes in~\cite{qasmi2025}. And the neighbour term in
Eq.~\eqref{eq:bcm-core} moves an agent towards the people it listens to,
following Deffuant--Weisbuch and
Hegselmann--Krause~\cite{deffuant2000,hegselmann2002}; the corresponding
expression in~\cite{qasmi2025} carries the opposite sign and moves agents
apart. We also avoid calling $\varepsilon$ a confirmation-bias
parameter, since a larger $\varepsilon$ means a wider tolerance and so
less confirmation bias, and the opposite reading has caused the same
result to be stated in two directions.

\subsection{Topics and Conditions}
\label{sec:conditions}

\paragraph{Choosing topics.}
One of our research questions asks how much the population's own
untouched trajectory shapes the apparent advantage of one side or the
other. Topics are therefore the unit of replication for that question,
and they have to differ in how the population drifts when nobody is
campaigning. We cannot know that in advance, so we screen candidates
first: each candidate claim is run briefly with no campaign agents, and
sorted by the direction and size of the resulting drift in mean stance.
From the screened pool we keep $n_{\mathrm{top}}$ claims covering
accepting, undecided and rejecting default positions. The claim whose
drift is closest to zero becomes the \emph{reference topic} and carries
the timing experiment, so that policy effects are measured where the
population pulls least in either direction and where the two sides have
similar room to move. Table~\ref{tab:topics} lists the selected claims.

\input{topics_table}

\paragraph{Conditions.}
Every topic is run under four conditions:
\begin{description}\itemsep2pt
  \item[\textsc{Null}] no campaign agents. This is not a control in the
    usual sense. It is the object one of our research questions is about:
    what the population does when left alone.
  \item[\textsc{\Prop-only}] the \prop{} alone, against that trajectory.
  \item[\textsc{\Chal-only}] the \chal{} alone, against that trajectory.
  \item[\textsc{Competition}] both sides, under a given pair of policies.
\end{description}
Every effect we report is a difference from the matching \textsc{Null}
run on the same topic, the same graph and the same personas.

\paragraph{Checking whether results depend on the population model.}
We re-run a subset of topics with the population model replaced by a
model of comparable ability from a different family, holding the probe,
the rater and everything else fixed. If an apparent advantage reflects
where the population model already stood rather than what the campaign
did, swapping the model should move it. We match the two models on
ability so that the comparison is between model families and not between
a strong model and a weak one.

\subsection{Measures}
\label{sec:measures}

Let $\bar{x}^{t}=\frac{1}{N}\sum_i x_i^{t}$. We report
\begin{align}
  \text{polarisation} \quad
  P^{t} &= \frac{1}{N}\sum_{i\in\mathcal{V}}
            \big(x_i^{t}-\bar{x}^{t}\big)^{2},
  \label{eq:polarisation}\\
  \text{advantage} \quad
  A^{t} &= \bar{x}^{t} - \bar{x}^{t}_{\textsc{Null}},
  \label{eq:advantage}\\
  \text{drift-corrected polarisation} \quad
  \Delta P^{t} &= P^{t} - P^{t}_{\textsc{Null}},
  \label{eq:dpol}
\end{align}
where Eq.~\eqref{eq:polarisation} is the measure used by Chitra and
Musco~\cite{chitra2020}. A positive $A^{t}$ means the \prop{} is ahead.
We also report the share of agents rejecting, undecided and accepting
($x\le-\tau$, $|x|<\tau$, $x\ge\tau$), and a persistence measure
\begin{equation}
  \rho_{\mathrm{pers}}
  = \frac{A^{T+T'}}{A^{T}},
  \label{eq:persistence}
\end{equation}
the share of the advantage held at the end of the campaign that is still
present after the quiet rounds.

The unit of replication is the run, not the agent. Every condition is
repeated $R$ times with a new graph, new personas and new random seeds,
and every quantity is reported as a mean over runs with a $95\%$
confidence interval. We obtain those intervals, and the smallest
difference the design can detect, by bootstrapping over runs. A
normal-theory formula is not appropriate here because the starting
distribution of opinions is deliberately spread out rather than
bell-shaped.

\subsection{Configuration}
\label{sec:config}

\begin{table}[t]
\centering
\small
\caption{Simulation parameters. Values marked $\dagger$ are held fixed
rather than varied.}
\label{tab:config}
\begin{tabular}{llr}
\toprule
Symbol & Meaning & Value \\
\midrule
$N$ & population agents & 30 \\
$\bar{d}$ & mean out-degree & 4 \\
$T$ & campaign rounds & 25 \\
$T'$ & quiet rounds & 8 \\
$B$ & budget per side (deliveries) & $\tfrac{1}{3}NT$ \\
$\ell$ & position length (tokens, at most) & 80 \\
$\lambda^{\dagger}$ & weight on the starting position & 0.3 \\
$w^{\dagger}$ & probability an addressed agent reads & 1.0 \\
$n_{s}^{\dagger}$ & posts shown to a campaign agent & 5 \\
$\tau$ & stance band cutoff & 0.5 \\
$k_{J}^{\dagger}$ & repeat ratings for rater validation & 5 \\
$\varepsilon$ & confidence threshold (numerical arm) & 0.3 \\
$\mu$ & convergence rate (numerical arm) & 0.3 \\
$n_{\mathrm{top}}$ & topics & 8 \\
$R$ & replicates per condition & 6--20 \\
\bottomrule
\end{tabular}
\end{table}

% ---------------------------------------------------------------
% NOTE ON REPLICATE COUNTS BELOW.
% The table encodes the post-top-up plan (Null R=20, Competition
% R=16, 482 runs). If the additional credit is not spent, the
% pre-top-up values are Null R=10 and Competition R=8, giving 338
% runs; the bootstrapped smallest detectable difference then rises
% from about 29-33% to about 41-46% of the polarisation level.
% Confirm after the calibration runs and update this table and the
% Scope and Limitations subsection together.
% ---------------------------------------------------------------
\begin{table}[t]
\centering
\small
\caption{Experimental blocks. The uniform--uniform competition cell is
shared between the timing experiment and the per-topic condition set at
the reference topic.}
\label{tab:blocks}
\begin{tabular}{llrr}
\toprule
Block & Cells & $R$ & Runs \\
\midrule
\textsc{Null}, per topic               & 8              & 20 & 160 \\
\textsc{\Prop-only}, per topic         & 8              & 6  & 48 \\
\textsc{\Chal-only}, per topic         & 8              & 6  & 48 \\
\textsc{Competition}, per topic        & 8              & 16 & 128 \\
Timing policies, reference topic       & 8              & 6  & 48 \\
Population-model check                 & $4\times2$     & 5  & 40 \\
Scale robustness ($N\!=\!100$)         & 2              & 5  & 10 \\
\midrule
\multicolumn{3}{l}{Total}                               & 482 \\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{tab:config} lists the parameters and Table~\ref{tab:blocks}
the experimental blocks. Four separate models are used: one for the
population, one for campaign message generation, one for rating messages,
and one for the stance probe. The probe comes from a different family
than the population, as Section~\ref{sec:measurement} requires. Model
identifiers, sampling temperatures and the prompts are given in the
appendix.

\subsection{Scope and Limitations}
\label{sec:limitations}

Four limitations follow from the design, and we state them here rather
than at the end.

First, the population is an artificial society and not a model of a human
one. Role-playing LLM populations behave differently from human groups,
including a tendency to agree with each other too
readily~\cite{chuang2025}. We treat the behaviour of this population as
the thing being studied, not as a stand-in for human opinion change.

Second, the campaign agents do not optimise. They choose what to say in
response to what they can observe, but their spending schedules are fixed
before the run and their targets are random. This study therefore maps
the outcomes produced by a set of policies; it does not show an agent
learning a policy. Finding out what an agent that adjusted its own
schedule would settle on is a natural next step, and it would require
giving that agent some view of the population's state.

Third, we do not study whom to target. Budget buys reach and target sets
are random, so our results speak to when money is spent and not to where
it is aimed. At $N=30$ a study of targeting by centrality or community
would in any case be dominated by which graph happened to be drawn; work
that puts targeting at its centre uses much larger
populations~\cite{dehkordi2026}.

Fourth, the design detects large effects only. With the replicate counts
in Table~\ref{tab:blocks}, the smallest difference between two conditions
that we can distinguish is in the region of $30$ to $50\%$ of the
polarisation level. We report the value we actually achieve alongside the
results, and we ask whether the timing of spending makes a large
difference rather than a subtle one.



==> results-old.tex <==
\section{Results}



\textcolor{red}{something is seriously wrong with placement of figures. Latex not rendering at the correct spot.}


\textcolor{red}{To be written again as the values may not match the results}

\subsection{RQ2: the uninfluenced trajectory and the apparent advantage}

Left alone, the population does not stay where it starts, and how far
it moves depends on the topic (Figure~\ref{fig:cross_topic}, left). The
drift over a run ranges from $-0.15$ on the MMR claim to $+0.15$ on
vaccines and child mortality, and in seven of eight topics its CI
excludes zero. The direction follows the epistemic standing of the
claim rather than the starting distribution, which is identical across
topics: populations drift toward rejecting false claims and toward
accepting well-supported ones, and barely move on contested ones. Any
comparison of campaign conditions that ignores this drift attributes it
to whichever side is being measured; on MMR, drift accounts for roughly
two fifths of the raw change in mean opinion under competition.

Once the drift is removed by differencing against the seed-matched
null, a campaign's effect also follows the claim rather than the side
that speaks (Figure~\ref{fig:cross_topic}, right). On the three false
claims every campaign condition sits at or below zero: on MMR the
\prop{} alone moves the population \emph{further} toward rejection
($-0.12$ $[-0.16,-0.07]$), as does the \chal{} alone ($-0.18$) and the
contest between them ($-0.20$). On the two well-supported claims every
condition sits above zero, including the \chal{} arguing against the
claim ($+0.08$ on nuclear safety, $+0.21$ on vaccines). Only on the
three contested claims do the two sides move the population in
opposite directions, and there the contest lands between them or near
zero. Figure~\ref{fig:exemplars} shows how these endpoints arise: on
MMR the movement is complete within five rounds and holds; on
decoupling the two sides separate steadily and the contest settles
between them; on vaccines all three conditions climb for the full
campaign and are still rising when it stops. In none of the eight
topics does the eight-round quiet period return the effect toward zero.





\subsection{RQ1: timing}

With the drift removed, the timing experiment on the reference topic
yields the payoff matrix of Figure~\ref{fig:payoff}. Timing matters,
but through the relation between the two schedules rather than through
either schedule alone. The \prop{}'s payoff is largest when the two
sides do not spend in the same rounds (early against late, $+0.15$;
late against sustained, $+0.13$) and smallest when they do (early
against early, $+0.06$; late against late, $+0.03$); the mean
off-diagonal payoff exceeds the mean on-diagonal payoff by $0.040$
$[0.005, 0.071]$ within matched seeds. Consequently the \prop{}'s best
reply is always to avoid the \chal{}'s schedule and the \chal{}'s is
always to match it, and the game has no pure-strategy equilibrium: in
$81\%$ of bootstrap resamples of the runs no cell is a best reply for
both sides. The sustained schedule, the only one studied in Qasmi et
al.~\cite{qasmi2025}, is never a best reply for either side. The
interpretation is that debunking is most effective when it arrives in
the same rounds as the claim it answers, and a claim is most effective
when it has the floor alone; what each side wants is therefore a
property of the other's schedule, and no fixed schedule is stable.

Last figure goes here:
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/figC_payoff_matrix.pdf}
\caption{Timing payoff matrix on the reference topic (growth--emissions
decoupling). All nine cells are two-sided contests: both sides are
active in every run with equal budgets of 250 message deliveries, and
cells differ only in each side's spending schedule --- \emph{early}
(rounds 1--9), \emph{sustained} (rounds 1--25) or \emph{late} (rounds
17--25). Rows give the \prop{}'s schedule, columns the \chal{}'s. Each
cell reports the \prop{}'s payoff --- the population's mean opinion
after the eight quiet rounds minus that of the no-campaign run on the
same network, personas and starting opinions --- as the mean over runs
with its 95\% bootstrap CI ($n{=}8$ per cell; $n{=}16$ for
sustained--sustained). $\blacktriangle$ marks the \prop{}'s best reply
to the \chal{}'s schedule in that column; $\blacktriangledown$ the
\chal{}'s best reply to the \prop{}'s schedule in that row. No cell
carries both: the \prop{} gains most when the schedules do not overlap
in time, the \chal{} when they coincide, so the game has no
pure-strategy equilibrium (absent in 81\% of bootstrap resamples).}
\label{fig:payoff}
\end{figure}
